An extended range of energy stable flux reconstruction methods on triangles

We present an extended range of stable flux reconstruction (FR) methods on triangles through the development and application of the summation-by-parts framework in two-dimensions. This extended range of stable schemes is then shown to contain the single parameter schemes of \citet{Castonguay2011} on triangles, and our definition enables wider stability bounds to be developed for those single parameter families. Stable upwinded spectral difference (SD) schemes on triangular elements have previously been found using Fourier analysis. We used our extended range of FR schemes to investigate the linear stability of SD methods on triangles, and it was found that a only first order SD scheme could be recovered within this set of FR methods.

==> conservation.tex <==
\section{Conservation}\label{sec:cons}
    General proofs for the conservation of the FR method can be performed irrespective of the flux function.  Hence, we will investigate conservation separately from any particular systems, such as will be important in the later proof of stability. Considering \cref{eq:cons_eq}, the first of two lemmas on this topic is
    \begin{lemma}[Linear conservation]\label{lem:lin_cons}
        Consider the $d$-dimensional FR method with linear flux function such that, for Banach space $V$, $\mathbf{u}\in V$ and $\mathbf{F} = F(\mathbf{u})\in (V^\prime,V)^d$, then sufficient conditions for conservation are that the gradient operator is are least first order accurate, \ie
        \begin{equation}\label{eq:sc_cond1}
            \mathbf{G1} = \mathbf{0},
        \end{equation}
        and that the lifting operator is such that
        \begin{equation}\label{eq:sc_cond2}
            \mathbf{1}^T\mathbf{MC} = \mathbf{1}^T\mathbf{L}^T_\partial\mathbf{W}_\partial.
        \end{equation}
    \end{lemma}
    \begin{proof}
        Let $\mathbf{u}_i=u(\mathbf{x}_i)$ and $\mathbf{F} = F(\mathbf{u})$, then the FR method can be written as
        \begin{equation}
            \dx{\mathbf{u}}{t} = -\mathbf{DF} - \mathbf{C}\left[(\mathbf{n}\cdot\mathbf{F})^\mathrm{num} - \mathbf{N}\hb{L}_{\partial}\mathbf{F}\right]
        \end{equation}
        Then multiplying by $\mathbf{1}^T\mathbf{M}$ we obtain
        \begin{equation*}
            \mathbf{1}^T\dx{}{t}\mathbf{Mu}= \dx{}{t}\mathbf{1}^T\mathbf{Mu} = -\mathbf{1}^T\mathbf{MDF} - \mathbf{1}^T\mathbf{MC}\left[(\mathbf{n}\cdot\mathbf{F})^\mathrm{num} - \mathbf{N}\hb{L}_{\partial}\mathbf{F}\right].
        \end{equation*}
        Then applying \cref{eq:sbp} we obtain
        \begin{equation*}
            \dx{}{t}\mathbf{1}^T\mathbf{Mu} = \mathbf{1}^T\mathbf{G}^T\hb{M}\mathbf{F} - \mathbf{1}^T\mathbf{L}_\partial^T\mathbf{W}_\partial\mathbf{N}\hb{L}_\partial\mathbf{F} - \mathbf{1}^T\mathbf{MC}\left[(\mathbf{n}\cdot\mathbf{F})^\mathrm{num} - \mathbf{N}\hb{L}_{\partial}\mathbf{F}\right].
        \end{equation*}
        If \cref{eq:sc_cond1} holds, then we obtain
        \begin{equation*}
            \dx{}{t}\mathbf{1}^T\mathbf{Mu} = - \mathbf{1}^T\mathbf{L}_\partial^T\mathbf{W}_\partial\mathbf{N}\hb{L}_\partial\mathbf{F} - \mathbf{1}^T\mathbf{MC}\left[(\mathbf{n}\cdot\mathbf{F})^\mathrm{num} - \mathbf{N}\hb{L}_{\partial}\mathbf{F}\right],
        \end{equation*}
        and proceeding to apply \cref{eq:sc_cond2} we get
        \begin{equation*}
            \dx{}{t}\mathbf{1}^T\mathbf{Mu} = - \mathbf{1}^T\mathbf{L}^T_\partial\mathbf{W}_\partial(\mathbf{n}\cdot\mathbf{F})^\mathrm{num}.
        \end{equation*}
        The term on the right-hand side is discrete statement of divergence theorem, which in 1D would give $f_R - f_L$. Therefore, the scheme is conservative. 
    \end{proof}
    
    Before moving onto the second lemma, we require the definition of an $L_2$ projection operator. 
    \begin{definition}[$L_2$ projection]\label{def:l2_proj}
        For a nodal point set $\{\pmb{\zeta}_i\}_{i\leq N_q}$ defining some polynomial basis $Q\in\mathbb{Q}_q$ with an associated quadrature $\{\pmb{\omega}_i\}_{i\leq N_q}$ of strength at least $2q-1$, and a point set $\{\mathbf{x}_i\}_{i\leq N_k}$ defining $R\in\mathbb{Q}_k$ such that $N_q > N_k$ and $q>k$, then the $L_2$ projection matrix from $Q$ to $R$ is then
        \begin{equation}
            \mathbf{R}_{qk} = (\mathbf{P}_{qk}^T\mathbf{M}_q\mathbf{P}_{qk})^{-1}\mathbf{P}_{qk}^T\mathbf{M}_q,
        \end{equation}
        where $\mathbf{P}_{qk}$ is the prolongation matrix that interpolates from $R$ to $Q$.
    \end{definition}
    
    This brings us the second lemma, non-linear conservation
    \begin{lemma}[Non-linear conservation]\label{lem:nlc}
        Consider the $d$-dimensional FR method with a non-linear flux function such that $F:(\mathbb{Q}_k) \mapsto W \subset (\mathbb{P}_q)^d$ for $q>k$. Then let if 
        \begin{equation}
            \mathbf{1}^T\mathbf{P}_{qk}^T\mathbf{M}_q\mathbf{P}_{qk}\mathbf{C} = \mathbf{1}^T(\mathbf{L}_\partial\mathbf{P}_{qk})^T\mathbf{W}_\partial
        \end{equation}
        provided the surface quadrature is sufficiently strong.
    \end{lemma}
    \begin{proof}
        The FR method with for a non-linear flux, restricted to the space $\mathbb{Q}_k$ can be written as:
        \begin{equation}
            \dx{\mathbf{u}}{t} = -\mathbf{D}\mathbf{R}_{qk}\mathbf{F}_q - \mathbf{C}\left[(\mathbf{n}\cdot\mathbf{F})^\mathrm{num} - \mathbf{N}\hb{L}_{\partial}\mathbf{R}_{qk}\mathbf{F}_q\right]
        \end{equation}
        If we multiply through by $\mathbf{1}^T\mathbf{P}_{qk}^T\mathbf{M}_q\mathbf{P}_{qk}$ then the proof follows that shown in \cref{lem:lin_cons}.
    \end{proof}
    \begin{remark}
        This lemma is similar to that presented by \citet{Chan2018}, and shows that when aliasing occurs with respect to the flux function, the scheme can still be conservative if a sufficiently strong quadrature is used to perform an $L_2$ projection of the solution.
    \end{remark}

==> tikz/do_not_delete.tex <==
%this directory is for the cached tikz figures, see  https://www.overleaf.com/learn/latex/Questions/I_have_a_lot_of_tikz,_matlab2tikz_or_pgfplots_figures,_so_I'm_getting_a_compilation_timeout._Can_I_externalise_my_figures%3F
